Polarization properties of FRB 20201124A from detections with the 100-m Effelsberg Radio Telescope

The repeating FRB source, FRB 20201124A, was found to be highly active in March and April 2021. We observed the source with the Effelsberg 100-m radio telescope at 1.36 GHz on 9 April 2021 and detected 20 bursts. A downward drift in frequency over time is clearly seen from the majority of bursts in our sample. A structure-maximizing dispersion measure (DM) search on the multi-component bursts in our sample yields a DM of 411.6$\pm$0.6 pc/cm$^3$. We find that the rotation measure (RM) of the bursts varies around their mean value of -605 rad/m$^2$ with a standard deviation of 11.1 rad/m$^2$. This RM magnitude is 10 times larger than the expected Galactic contribution along this line of sight (LoS). We estimate a LoS magnetic field strength of 4--6 $\mu$G, assuming that the entire host galaxy DM contributes to the RM. Further polarization measurements will help determine FRB 20201124A's RM stability. The bursts are highly linearly polarized, with some showing signs of circular polarization, the first for a repeating FRB. Their polarization position angles (PAs) are flat across the burst envelopes and vary between bursts. We argue that the varying polarization fractions and PAs of FRB 20201124A are similar to known magnetospheric emission from pulsars, while the observed circular polarization, combined with the RM variability, is hard to explain with Faraday conversion. The high linear polarization fractions, flat PAs, and downward drift from FRB 20201124A bursts are similar to previous repeating sources, while the observed circular polarization is a newly seen behaviour among repeaters.

==> makefile <==
SHELL:=/bin/bash
all:main.tex
	latexmk -pdf -silent 

debug:main.tex
	latex $< ;\
	open main.pdf &

old:main.tex
	latex $< ;\
	bibtex rm ;\
	latex $< ;\
	latex $< ;\
	pdflatex $< ;\
	open main.pdf &

.PHONY: gadd
gadd:
	@read -p "git commit description: " DESCRIPTION;\
	git add . ;\
	git commit -m "$$DESCRIPTION" 

.PHONY: gpush
gpush:
	git push origin;

gpull:
	@read -p "remote name:" REMOTE;\
	git pull $$REMOTE master --allow-unrelated-histories

gcheck:
	git log -p -2

gremote:
	git remote add overleaf $$URLoverleaf
	git remote add github $$URLgithub

.PHONY: clean
clean: 
	rm -f *.dvi  *.aux *.blg *.toc *.out *.fdb_latexmk *.log *.synctex.gz *.fls

